Automated Correction for Syntax Errors in Programming Assignments using Recurrent Neural Networks

We present a method for automatically generating repair feedback for syntax errors for introductory programming problems. Syntax errors constitute one of the largest classes of errors (34%) in our dataset of student submissions obtained from a MOOC course on edX. The previous techniques for generating automated feed- back on programming assignments have focused on functional correctness and style considerations of student programs. These techniques analyze the program AST of the program and then perform some dynamic and symbolic analyses to compute repair feedback. Unfortunately, it is not possible to generate ASTs for student pro- grams with syntax errors and therefore the previous feedback techniques are not applicable in repairing syntax errors. We present a technique for providing feedback on syntax errors that uses Recurrent neural networks (RNNs) to model syntactically valid token sequences. Our approach is inspired from the recent work on learning language models from Big Code (large code corpus). For a given programming assignment, we first learn an RNN to model all valid token sequences using the set of syntactically correct student submissions. Then, for a student submission with syntax errors, we query the learnt RNN model with the prefix to- ken sequence to predict token sequences that can fix the error by either replacing or inserting the predicted token sequence at the error location. We evaluate our technique on over 14, 000 student submissions with syntax errors. Our technique can completely re- pair 31.69% (4501/14203) of submissions with syntax errors and in addition partially correct 6.39% (908/14203) of the submissions.

==> orig_motivation_examples.tex <==
\begin{figure*}
\begin{tabular}{|c c|}
\hline
\multicolumn{2}{c}{\bf SyntaxError - Insert Token}\\
\hline
\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recPower(base, exp):
    if exp <= 0:
        return 1
    return base * recPower(base, exp - 1    
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recPower(base, exp):
    if exp <= 0:
        return 1
    return base * recPower(base, exp - 1)    
\end{python}
}
\end{minipage}
\\ \hline
\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recPower(base, exp):
    if exp <= 0:
        return 1
    return base * recPower(base, exp-)    
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recPower(base, exp):
    if exp <= 0:
        return 1
    return base * recPower(base, exp - 1)    
\end{python}
}
\end{minipage}
\\ \hline
\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recPower(base, exp):
    if exp == 1:
        return base
    return base * (recPower(base, (exp - 1))    
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recPower(base, exp):
    if exp == 1:
        return base
    return base * (recPower(base, (exp - 1)))    
\end{python}
}
\end{minipage}
\\ \hline

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recPower(base, exp):
    if exp > 1:
        return base * recurPower(base, exp-1)
    else
        return 1
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recPower(base, exp):
    if exp > 1:
        return base * recurPower(base, exp-1)
    else:
        return 1
\end{python}
}
\end{minipage}
\\\hline

\multicolumn{2}{c}{\bf SyntaxError - Replace Token}\\
\hline
\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 0:
        return 1
    return base = recurPower(base,exp-1)
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 0:
        return 1
    return base * recurPower(base,exp-1)  
\end{python}
}
\end{minipage}
\\ \hline

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if(exp==0):
        return sum
    else:
        sum*=base
        return sum+recurPower(base,exp-=1)
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if(exp==0):
        return sum
    else:
        sum*=base
        return sum+recurPower(base,exp-11)
\end{python}
}
\end{minipage}
\\ \hline

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp=0:
      return 1;
    else
      return base*recurPower(base,exp-1)
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp==0:
      return 1;
    else
      return base*recurPower(base,exp-1)
\end{python}
}
\end{minipage}
\\ \hline


\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 0:
        return 0
    elif exp == 1:
        return base
    else:
        return base * recurPower(base, exp - 1))
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 0:
        return 0
    elif exp == 1:
        return base
    else:
        return base * recurPower(base, exp - 1)
\end{python}
}
\end{minipage}
\\ \hline

\multicolumn{2}{c}{\bf SyntaxError - Previous Line Insert}\\
\hline

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    f exp == 1:
        return base
    return base * recurPower(base, (exp - 1))
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 1:
        return base
    return base * recurPower(base, (exp - 1))
\end{python}
}
\end{minipage}
\\ \hline

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 1:
        return base
    else:
        retrun base * recurPower(base, exp - 1)
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 1:
        return base
    else:
        return base * recurPower(base, exp - 1)
\end{python}
}
\end{minipage}
\\ \hline

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 1:
        return = exp
    else:
        return (base * recurPower(base, exp-1))
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 1:
        return base
    else:
        return (base * recurPower(base, exp-1))
\end{python}
}
\end{minipage}
\\ \hline


\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 0:
        return 1
    if exp == 1:
        return base
    if exp > 1:
        return exp -= 1
    else:
        return recurPower(base,exp-1)
\end{python}
}
\end{minipage}

&

\begin{minipage}{0.5\linewidth}
{\scriptsize
\begin{python}
def recurPower(base, exp):
    if exp == 0:
        return 1
    if exp == 1:
        return base
    if exp > 1:
        return base * recurPower(base,exp-1)
    else:
        return recurPower(base,exp-1)
\end{python}
}
\end{minipage}
\\ \hline

\end{tabular}
\end{figure*}


